Multi-Satellite MIMO Systems for Direct User-Satellite Communications: A Survey

Advancements in satellite technology have made direct-to-device connectivity a viable solution for ensuring global access. This method is designed to provide internet connectivity to remote, rural, or underserved areas where traditional cellular or broadband networks are lacking or insufficient. This paper is a survey providing an in-depth review of multi-satellite Multiple Input Multiple Output (MIMO) systems as a potential solution for addressing the link budget challenge in direct user-satellite communication. Special attention is given to works considering multi-satellite MIMO systems, both with and without satellite collaboration. In this context, collaboration refers to sharing data between satellites to improve the performance of the system. This survey begins by explaining several fundamental aspects of satellite communications (SatComs), which are vital prerequisites before investigating the multi-satellite MIMO systems. These aspects encompass satellite orbits, the structure of satellite systems, SatCom links, including the inter-satellite links (ISL) which facilitate satellite cooperation, satellite frequency bands, satellite antenna design, and satellite channel models, which should be known or estimated for effective data transmission to and from multiple satellites. Furthermore, this survey distinguishes itself by providing more comprehensive insights in comparison to other surveys. It specifically delves into the Orthogonal Time Frequency Space (OTFS) within the channel model section. It goes into detail about ISL noise and channel models, and it extends the ISL section by thoroughly investigating hybrid FSO/RF ISLs. Furthermore, analytical comparisons of simulation results from these works are presented to highlight the advantages of employing multi-satellite MIMO systems.

==> Biography.tex <==
% Author biographies
\IEEEbiography[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ZohrePhoto.jpg}}]{Zohre Mashayekh Bakhsh}{Zohre Mashayekh Bakhsh completed her B.Sc. degree in Electrical Engineering - Telecommunication at Babol Nooshirvani University of Technology, Iran, in 2015. She pursued her master's degree at K.N. Toosi University of Technology, Iran, focusing on the application of beamforming in cognitive radio systems and MIMO relay networks. Currently, she is a Ph.D. student at the 6GIC of the University of Surrey, where her research revolves around multi satellite MIMO systems. Her research interests encompass Satellite Communications (SatComs), MIMO technology, and Wireless Communications.}
%\IEEEbiography[<photo options>]{Yasaman Omid}{Biography text for Author 2.}
% \IEEEbiography[<photo options>]{Farbod Kayhan}{Biography text for Author 3.}
% \IEEEbiography[<photo options>]{Yi Ma}{Biography text for Author 3.}
% \IEEEbiography[<photo options>]{Rahim Tafazolli}{Biography text for Author 3.}
